Learning Category-Level Manipulation Tasks from Point Clouds with Dynamic Graph CNNs

This paper presents a new technique for learning category-level manipulation from raw RGB-D videos of task demonstrations, with no manual labels or annotations. Category-level learning aims to acquire skills that can be generalized to new objects, with geometries and textures that are different from the ones of the objects used in the demonstrations. We address this problem by first viewing both grasping and manipulation as special cases of tool use, where a tool object is moved to a sequence of key-poses defined in a frame of reference of a target object. Tool and target objects, along with their key-poses, are predicted using a dynamic graph convolutional neural network that takes as input an automatically segmented depth and color image of the entire scene. Empirical results on object manipulation tasks with a real robotic arm show that the proposed network can efficiently learn from real visual demonstrations to perform the tasks on novel objects within the same category, and outperforms alternative approaches.

==> porposedJunchiWriteup.tex <==
\begin{figure}[t]
  \centering
 {
    \includegraphics[width=0.46\textwidth]{images/door_example.pdf}
 }
\caption{Scene of opening a door. There are many region in the workspace, a robot need to locate relevant region, the card reader in this example, to unlock the door.}
 \label{fig:door_example}
 \vspace{-0.5cm}
\end{figure}

\section{Proposed Approach}

The proposed approach initially assumes that there are no hidden variables, and incrementally creates new ones only when needed to explain stochasticity of outputs. 

In this work, we focus on reward estimation in POMDP. Meanwhile, we investigate POMDP problems where hidden part of states can be inferred from the history of observable states. Further, proposed approach models hidden variables as whether a trajectory visits specific regions. It well fits tasks with topological structures where optimal behaviors can be divided into multiple stages, and each stage is characterized by traversing a subregion in observable state space. Proposed method aims at discovering most relevant regions for reward estimation.

We model subregion for hidden variable $M^i$ as a hyper-sphere: $(z-C^i)^2 \leq (\epsilon^i)^2$ ,with center $[C^i]^m_{i=1}$ and size $[\epsilon^i]^m_{i=1}$. So we can define hidden variable as $M^i(D_l)=I_{min_h (z^l_h - C^i)^2 \leq (\epsilon^i)^2}$ where $I_{condition}$ is the indicator function, a hidden variable is activated when the trajectory traverses this region.

To find most relevant memory, we measure information gains from these hidden variables on rewards, we start with one hidden variable and extend it to multiple case later: $IG(M) = H(R) - H(R|M)$ where $H(\cdot)$ is entropy and $H(\cdot|\cdot)$ is conditional entropy. To reduce uncertainty in reward prediction, we maximize the information gain over hidden variable $M$. As the first term is not related to $M$, the maximization is equivalent to minimizing $H(R|M)$. We assume rewards are discrete in the computation of entropy, which is true in many robotics application as a constant reward is provided only when a final goal is reached. In some continuous cases, after clustering reward values, the same computation can still be applied. The conditional entropy is defined as


\begin{eqnarray*}
H(R|M) = \sum_{r_k}\Big(-P(M=0,R=r_k)log \frac{P(M=0, R=r_k)}{P(M=0)} \\
      -P(M=1,R=r_k)log \frac{P(M=1, R=r_k)}{P(M=1)}\Big) \\
       = \, P(M=0)logP(M=0)+P(M=1)logP(M=1) \\
       -\sum_{r_k} \Big(P(M=0, R=r_k)log P(M=0, R = r_k) \\
       + P(M=1, R = r_k) log P(M=1, R = r_k)\Big)
\end{eqnarray*}

 where reward $R \in \{r_1 ... r_k\} $. From the last format of the conditional entropy, we can see, in ideal case - when a hidden variable completely determines a binary value reward, the conditional entropy decreases to zero as there exist a combination of values $(\mu, r)$ such that $P(M=\mu)=P(M=\mu, R=r)$. It shows that optimizing this conditional entropy can locate the most informative region.
 
Given the trajectory set $D$, a common way to estimate probability will be counting frequencies: $P(M=1) = \frac{ \Vert M=1 \Vert}{L} = \frac{1}{L} \sum^L_{l=1} I_{min(z^l-C)^2 \leq \epsilon^2}$. Plug this counting back to the conditional entropy, our goal becomes $\underset{C, \epsilon}{min} H(R|M)$. To take advantage of modern gradient descent based optimization tools, the objective function has to be differentialble. However, the indicator function does not satisfy the requirement. To covert this indicator counting into differentiable function, we use sigmoid function to replace the indicator function: $g(z^l, C, \epsilon) = \frac{1}{1+e^{\alpha[min(z^l-C)^2-\epsilon^2]}}$ where $\alpha$ is a positive constant. As $alpha$ is positive, $g(z^l, C, \epsilon)$ will get close to one when the trajectory's distance to the region center $C$, which is measured by the point cloest to the center along the trajectory, becomes smaller the radius $\epsilon$. On the other hand, it will move to zero when the trajectory is far from the region center. Though sigmoid function is differentiable, it is vulnerable to saturation issue. Small $alpha$ can alleviate this problem while introducing more bias as it become less similar with indicator function. So instead of keeping a fixed constant, we start from small $alpha$ and gradually increase it during training.

The extension to multiple hidden variables follows naturally. Replacing binary terms by enumerating combination of all hidden variables, we can get


\begin{align*}
&H(R|M^1...M^m)\\ 
       =& \, \sum_{\mu^1...\mu^m}[P(\mu^1...\mu^m)logP(\mu^1...\mu^m)\\
       &-\sum_{r_k} P(\mu^1...\mu^m, r_k)log P(\mu^1...\mu^m, r_k)]
\end{align*}

with $P(M^1=\mu^1...M^m=mu^m)$ as $P(\mu^1...mu^m)$ and $P(M^1=\mu^1...M^m=mu^m,R=r_k)$ as $P(\mu^1...mu^m, r_k)$. Similar with the single variable situation, this conditional entropy reaches zero when a combination of hidden variable matches a specific reward value. As what we do above, the indicator function inside this conditional entropy is substituted by sigmoid functions, but instead of using only one sigmoid function, we need product of sigmoid functions and each of them corresponds to one region. However, optimizing multiple regions simultaneously is difficult. We optimize these regions iteratively here: starting from single case above, in every iteration we locate next hidden region with found hidden variable. So in counting frequencies, we have sigmoid function for hidden variable being optimized and keep indicator function for found variable, i.e. $g(z^i, C^i, \epsilon^i)I_{z^{i-1},C^{i-1}, \epsilon^{i-1}}...I_{z^{1},C^{1}, \epsilon^{1}}$ in $i$-th iteration.

\begin{figure}
  \centering
 {
    \includegraphics[width=0.46\textwidth]{images/trajectory.pdf}
 }
\caption{Training trajectories in the {\it learning-to-paint} experiment collected with a random exploration policy. Red plots correspond to successful trajectories, blue plots correspond to failed trajectories. Successful trajectories are ones where the brush attached to the end-effector visits a special region of the workspace that corresponds to the paint bucket. Notice that it is hard to locate that region visually. The proposed algorithm successfully locate that region from information gains.}
 \label{fig:trajectory}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.46\textwidth]{images/kde_illustration.pdf}
    \caption{Regions with more trajectories have higher density estimation and hence get more sample points.}
    \label{fig:my_label}
\end{figure}

Even the objective function is differentiable, optimizing it is still nontrivial. But in many robotics tasks, all successful trajectories should more or less meet at those regions we try to discover. It motivates us to sampling from these trajectories rather than completely random generate initial parameters. We apply kernel density estimation with Gaussian kernel using states inside successful trajectories. A number of states in these trajectories are sampled and ranked according to their density estimation, the best one is chosen to be the starting point for $C$. In the case where there is multiple hidden variables, after sampling states, states inside previously found region are filtered out. The complete algorithm is described in Algorithm \ref{algo:discover_hidden}.

\begin{algorithm}
\KwIn{$m$ = Number of hidden variables, $n_restart$ = Number of optimization restart, and sampled data trajectories $\mathcal{D} = \{(z^l_0,a^l_0, \dots,z^l_h,a^l_h)\}_{l=1}^{L}$;}
\KwOut{Set of memory variables $\{M^i\}_{i=1}^{m}$}
$M \leftarrow \{\}$\;
\For{$i:=1; i\leq m; i \leftarrow i+1$}
{
    $candidate \leftarrow \{\}$\;
    \For{$j:=1; j \leq n_restart; j \leftarrow j+1$}
    {
        get $C^{(0)}_{i,j}$ from kernel density estimation based sampling, $\epsilon^{(0)}_{i,j}$ from uniform sampling\;
        $C*_{i,j}$, $\epsilon*_{i,j} = argmin H(R|M^1...M^i)$ \;
        $candidate \leftarrow candidate \cup (C*_{i,j}, \epsilon*_{i,j}, H(R|M^1...M^{i-1}), C*_{i,j}, \epsilon*_{i,j}) $ \;
    }
    $M \leftarrow M \cup best\ candidate$
}
\caption{Discover Hidden Variables}
\label{algo:discover_hidden}
\end{algorithm}
